A new Simheuristics procedure for stochastic combinatorial optimization

Ignoring uncertainty in combinatorial optimization leads to suboptimal decisions in practice. Nevertheless, the focus is often on deterministic combinatorial optimization problems, mainly because they are already challenging enough without stochasticity. To make it easier to address stochasticity in combinatorial optimization, Simheuristics have been developed that allow solving stochastic combinatorial optimization problems. We propose a new Simheuristic procedure that dynamically changes the optimization focus between a deterministic and stochastic perspective based upon a statistical model. By doing so, an adequate trade-off is made between exploration and exploitation of the solution space during the optimization. We numerically show that the new Simheuristic procedure solves real-life stochastic scheduling problems more efficiently than standard Simheuristics strategies.

==> Macros/SNELatexTemplateMacrosVol23plus__Markus_Wallerbergers_in_Konflikt_stehende_Kopie_2015-06-03_.tex <==
 %% use these commands to change font, fontstyle and fontsize 
%% \sfdefault ... OpenSans, \rmdefault ... Times Roman, \ttdefault ... Courier
%\usefont{T1}{\sfdefault}{bx}{n}}
%\fontsize{5cm}{1em}\selectfont 

%% set standard fonts
\renewcommand*\rmdefault{ptm}  % standard roman-font
\renewcommand*\ttdefault{pcr}  % standard type-writer-font
\renewcommand*\familydefault{\rmdefault} % default-font is roman-font

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% format/layout - parameter:
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
%\setlength{\parskip}{0.05\baselineskip}
\setlength{\parindent}{5mm}

\geometry{
     includeall,
     asymmetric, 
     bindingoffset=0mm,
     inner=21mm,
     outer = 21mm,
     nomarginpar,
     top=18.2mm,      
     headheight=4.3mm,
     headsep = 9.3mm,
     bottom=34.2mm, %30.9
     %height = 247.3mm
     footskip = 10mm,     
     columnsep=8mm,      
}

% resolution
\pdfpxdimen=1in
\divide\pdfpxdimen by 600

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% custom color - definition:
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{SNE_DARK_BLUE}{RGB}{23, 54, 93} % used for Title
\definecolor{SNE_BLUE}{RGB}{30, 72, 124} % used section and subsection headlines, paragraph-headlines, Abstract,..
\definecolor{SNE_BRIGHT_BLUE}{RGB}{54, 94, 144} % used for header and footer
\definecolor{SNE_GRAY}{RGB}{77,77,77} % used for box with doi-number

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setcounter{page}{\value{startpage}}

\newcounter{ct}
\newcounter{ct2}
\newcommand{\addspaces}[1]{%
  \StrLen{#1}[\abc]
  \setcounter{ct}{\abc}
  \stepcounter{ct}
  \setcounter{ct2}{1}
  \whiledo{\value{ct} > 1}%
  {%
	\StrMid{#1}{\value{ct2}}{\value{ct2}}[\char]%
	\IfEq{\char}{ }{\hspace{1.7mm}}{\char\hspace{1.5mm}}%
	\stepcounter{ct2}%
	\setcounter{ct}{\value{ct}-1}%
   }
}

\newlength{\HSpaceLength}
\newcommand{\HSpaceOfText}[1]{\settowidth{\HSpaceLength}{#1}\hspace{\HSpaceLength}}

\makeatletter
\def\hlinewd#1{%
\noalign{\ifnum0=`}\fi\hrule \@height #1 %
\futurelet\reserved@a\@xhline}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% configure style of headings, capture-text, ...
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\allowdisplaybreaks[4] % page break within align-environment 0...4 priority   

\renewcommand\figurename{\footnotesize\fontsize{8.1pt}{1em}\sf\bfseries Figure} %% Name of figures. Change to "Abbildung" if document is written in German.
\renewcommand\tablename{\footnotesize\fontsize{8.1pt}{1em}\sf\bfseries Table} % Name of tables. Change to "Tabelle" if document is written in German.
\renewcommand{\refname}{\sf\bfseries\normalsize References}

\addtokomafont{subsection}{\color{SNE_BLUE}} %\usefont{T1}{\sfdefault}{bx}{n}}}
\addtokomafont{subsection}{\sf\bfseries}
\addtokomafont{subsection}{\normalsize}
\addtokomafont{section}{\sf\bfseries}
\addtokomafont{section}{\color{SNE_BLUE}}
\addtokomafont{section}{\Large\fontsize{14.1pt}{1em}\selectfont}
\addtokomafont{paragraph}{\sf\bfseries}
\addtokomafont{paragraph}{\color{SNE_BLUE}}
\addtokomafont{paragraph}{\normalsize}
\newcommand{\Abstract}[1]{\paragraph{\small\fontsize{8.7pt}{1em}\selectfont\sf\bfseries Abstract.}{\small\fontsize{8.7pt}{1em}\selectfont\sf #1}}
\addtokomafont{caption}{\sf}
\addtokomafont{caption}{\setstretch{1.3}}
\addtokomafont{caption}{\footnotesize\fontsize{8.1pt}{1.2em}\selectfont}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% title-section - definition:
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\maketitle}{
\twocolumn[\vspace{-3mm}{\sf
  {\setstretch{2.36}
    \begin{center}
      {\textcolor{SNE_DARK_BLUE}{\bfseries\huge\fontsize{19.3pt}{1em}\selectfont \papertitle}}\\
      \vspace{-0.4mm}
      {\large\fontsize{12.2pt}{1em}\selectfont \authors}
    \end{center}
  }\vspace{-0.3mm}    
  {\setstretch{1}
    {\small\fontsize{9.1pt}{1em}\selectfont \institutes }
  }}
  \vspace{7.05mm}
]
}
\setcounter{page}{1}
